Integrated Bundling and Pricing of Unique Items

Retailers have significant potential to improve recommendations through strategic bundling and pricing. By taking into account different types of customers and their purchasing decisions, retailers can better accommodate customer preferences and increase revenues while reducing unsold items. We consider a retailer seeking to maximize its expected revenue by selling unique and non-replenishable items over a finite horizon. The retailer may offer each item individually or as part of a bundle. Our approach provides tractable bounds on expected revenue that are tailored to unique items and suitable for a rich class of choice models. We leverage these bounds to propose a bundling algorithm that efficiently selects bundles in a column-generation fashion. Under the multinomial logit model, our bounds are asymptotically optimal as the expected number of arrivals $\lambda$ grows, yielding a performance bound in $O(1/\lambda)$. In contrast, we show that both the static and fluid approximations are not asymptotically optimal. Moreover, we propose a greedy algorithm that allows for tractable dynamic bundling. We show through numerical experiments that third-party logistics providers (3PL) in particular can benefit from improved load recommendations and pricing decisions. By not only minimizing shipping costs, but also reducing empty miles and suggesting options that better match carrier preferences, our methodology benefits digital brokerage platforms while contributing to the transportation industry's sustainability efforts. In a Texas Triangle simulation powered by Uber Freight data, dynamic bundling and pricing reduces costs by 6%, empty miles by 25%, and more than halves the number of unmatched loads over dynamic pricing alone.

==> 5_CG_Bundling_Alg.tex <==
\section{Bundling Algorithm} \label{section:Bunlding}

Now that we have established some tools for evaluating the performance of a given set of options, we turn our attention to problem \eqref{eq:first_stage} i.e. we want to find the set of options $S$ that maximizes $V_{T(\ear)}^*(S)$ for a fixed $\ear$. As explained in the introduction, this problem is computationally challenging. However, by leveraging the bounds outlined in Section \ref{section:bounds}, we can now effectively assess the performance of a given set of options. Consequently, we focus our efforts on identifying the set that minimizes the optimality gap instead of the set maximizing the exact expected revenue.

The main challenges in finding the set maximizing the DFA are that $V^\text{DFA}_{T(\ear)}$ is a non-linear set function and that the cardinality of the search space explodes as $L$ increases. Indeed, there are $L!/2^{\lfloor L/2 \rfloor}$ ways to partition $\mathcal{L}$ into ordered pairs. Thus we obtain $|\mathcal{P}(\mathcal{L})| \geq L!/2^{\lfloor L/2 \rfloor} \geq \frac{1}{2}\left(\frac{L}{e\sqrt{2}}\right)^L$ and $\mathcal{P}(\mathcal{L})$ grows exponentially in $L$. Further, the cardinality of $\mathcal{O}$ is in the order of $L^K$, making $|\mathcal{O}|$ large enough to prevent evaluating the DFA bound of each option in $\mathcal{O}$. This section addresses these challenges by developing an algorithm that efficiently explores bundles and forms a set of options aiming to minimize the optimality gap. This algorithm involves three major steps:
\begin{enumerate}
    \item Compute the individual upper bound $u_{T(\ear),i}$ for all $i \in \mathcal{O}$.
    \item Linearize the contribution of each option to $V^\text{DFA}_{T(\ear)}$ and form a set partitioning problem. Relax the binary constraints of this problem and solve it in a column-generation fashion using perturbed reduced costs.
    \item Obtain multiple solutions to the set partitioning problem with binary constraints, evaluate their DFA bounds, and select the one achieving the largest bound.\\
\end{enumerate}

Recall that the optimistic bound $V^U_{T(\ear)}(S)$ of a set of options $S$ is the sum of the contributions $u_{T(\ear),i}$ of each option it contains, which can be computed in parallel. Therefore, it is sufficient to determine the individual upper bound $u_{T(\ear),i}$ of each option $i$ to retrieve the upper bound of any set of options easily.

Let $S_0$ be the of singletons i.e. the set of options containing single products only, and $S_i$ be the set containing option $i$ and all single products not included in option $i$. We linearize the contribution of each option to the DFA of any set by letting $r_i = V_{T(\ear)}^\text{DFA}\left(S_i\right) - V_{T(\ear)}^\text{DFA}\left(S_0\right)$ be the DFA improvement of option $i$. We then consider the following set partitioning problem:
\begin{align*}
    \max_{z} & \sum_{i \in \mathcal{O}} z_i r_i \tag{$\mathcal{P}_{IO}$}\\
    \text{s.t.} & \sum_{i \in \mathcal{O}\;:\;l \in i} z_i = 1, \quad \forall l \in \mathcal{L}\\
    &\sum_{i \in \mathcal{O}\;:\;\#i > 1} z_i \leq K_s,\\
    &z_i \in \{0,1\}, \quad \forall i \in \mathcal{O}
\end{align*}
where $\#i$ is the cardinality of option $i$ i.e. the number of products it contains.

Problem $\mathcal{P}_{IO}$ consists of selecting the partition of $\mathcal{L}$ maximizing the total DFA improvement. The first constraint ensures that the solution of $\mathcal{P}_{IO}$ is a partition of $\mathcal{L}$, and the second ensures that the solution is binary. By relaxing the latter constraints, we obtain a linear program whose primal and dual formulations are given below:

\begingroup
\vspace{-0.6cm}
\centering
\begin{minipage}[t]{.49\linewidth}
\begin{align*}
    \max_{z} & \sum_{i \in \mathcal{O}} z_i r_i \tag{$\mathcal{P}_{LP}$}\\
    \text{s.t.} & \sum_{i \in \mathcal{O}\;:\;l \in i} z_i = 1, \quad \forall l \in \mathcal{L}\\
    &\sum_{i \in \mathcal{O}\;:\;\#i > 1} z_i \leq K_s,\\
    &z_i \in [0,1], \quad \forall i \in \mathcal{O}\\
\end{align*}
\end{minipage}%
\begin{minipage}[t]{.49\linewidth}
\begin{align*}
    \min_{\mu} & \sum_{l \in \mathcal{L}} \mu_l + \sum_{i \in \mathcal{O}} \mu_i + \mu_{K_s}\tag{$\mathcal{P}_{D}$}\\
    \text{s.t.} & \sum_{l\in i} \mu_l + \mu_i + \mu_{K_s} \mathds{1}_{\{\#i>1\}} \geq r_i, \quad \forall i \in \mathcal{O}\\
    &\mu_i \geq 0, \quad \forall i \in \mathcal{O}\\
    &\mu_{K_s} \geq 0
\end{align*}
\end{minipage}
\endgroup

\noindent where $\mu_l$ is the dual variable associated to the $l$-th constraint of the primal problem, $\mu_i$ the dual variable associated to the constraint $z_i \leq 1$, and $\mu_{K_s}$ is the dual variable associated to the last constraint of the primal problem. This relaxation allows us to form high-potential bundles in a column-generation fashion. The master problem is defined as $\left(\mathcal{P}_{LP}\right)$ except that the set $\mathcal{O}$ is restrained to $\overline{\mathcal{O}}$. Initially, the restained set contains all single products i.e. $\overline{\mathcal{O}} = \mathcal{L}$.

At each iteration, we solve the master problem to obtain the primal and dual optimal solutions $(z^*, \mu^*)$. Ideally, we then add to the master problem the option not already included in $\overline{\mathcal{O}}$ with the largest reduced cost $\overline{r}_i = r_i - \sum_{l \in i} \mu^*_l - \mu^*_{K_s}$. However, by the definition of $r_i$, this would require computing $V_{T(\ear)}^\text{DFA}\left(S_i\right)$ for all $i \in \mathcal{O}$ which can be computationally expensive. Instead, we remark that $\overline{r}_i \leq \tilde{r}_i \triangleq V^U_{T(\ear)}(S_i) - V_{T(\ear)}^\text{DFA}\left(S_0\right) - \sum_{l \in i} \mu^*_l - \mu^*_{K_s}$. Let $i^* = \argmax_{i} \tilde{r}_i$. If $\tilde{r}_{i^*} > 0$, option $i$ is added to $\overline{\mathcal{O}}$. Otherwise, as $\tilde{r}_{i^*} \leq 0$ implies $\max_{i} \overline{r}_i \leq 0$, no option has a positive reduced cost and the generation of bundles stops. Since the number of iterations to obtain non-positive reduced costs can be large, we limit the number of generated options to $N_\text{gen}$.

We then restore the binary constraints and solve $\left(\mathcal{P_{IO}}\right)$ using the set of promising options $\overline{\mathcal{O}}$. Note that the revenue improvement $r_i$ simply compares the quality of the DFA bounds of $S_i$ and $S_0$ so it does not capture the interaction between options. Therefore, solving $\left(\mathcal{P_{IO}}\right)$ over $\overline{\mathcal{O}}$ can produce solutions suffering from this lack of information. Instead, we generate a set $\mathcal{S}$ of up to $N_\text{eval}$ solutions to $\left(\mathcal{P_{IO}}\right)$ over $\overline{\mathcal{O}}$ by sequentially solving and constraining problem $\left(\mathcal{P_{IO}}\right)$ to prevent selecting any previous solution. We then evaluate $V_{T(\ear)}^\text{DFA}\left(S\right)$ for all $S \in \mathcal{S}$, and select the set achieving the largest value. The bundling algorithm is described in Algorithm \ref{alg:bld_alg}.

Additionally, we note that the upper bound $V^U_{T(\ear)}(S)$ of a set of options is linear in the individual upper bounds $u_{T(\ear),i}$ of each option it contains. Thus, one can easily compute the set $S^*$ achieving the largest upper bound using the individual upper bounds $u_{T(\ear),i}$ obtained in the first loop of Algorithm \ref{alg:bld_alg} by solving the following MILP:
\begin{align*}
    \max_{z} & \sum_{i \in \mathcal{O}} z_i \cdot u_{T(\ear),i}\\
    \text{s.t.} & \sum_{i \in \mathcal{O}\;:\;l \in i} z_i = 1, \quad \forall l \in \mathcal{L}\\
    &\sum_{i \in \mathcal{O}\;:\;\#i > 1} z_i \leq K_s,\\
    &z_i \in \{0,1\}, \quad \forall i \in \mathcal{O}
\end{align*}
The largest upper bound $V^U_{T(\ear)}(S^*)$ can then be used to compute the optimality gap of the solution returned by Algorithm \ref{alg:bld_alg}.

\begin{algorithm}
\caption{Bundling Algorithm}\label{alg:bld_alg}
\begin{algorithmic} \small
\Require $\mathcal{L}$: set of products, $K_s$: maximum number of bundles, $K_b$: maximum bundle size
\State $\mathcal{O} \leftarrow \left\{(l_1, \hdots, l_k) \in \mathcal{L}^k\;|\; k\leq K_b \text{ and } l_a \neq l_b, \text{ for } a\neq b\right\}$  \Comment{$\mathcal{O}$ is the set of all options of size at most $K_b$}
\For{$i \in \mathcal{O}$}
    \State Compute $\left(u_{t,i} , \tau^U_{t,i}\right)_{t \in [T(\ear)]}$
\EndFor
\State $\overline{\mathcal{O}} \leftarrow \left\{i \in \mathcal{O} \;|\;\#i=1\right\}$
\Do
\State Solve master problem to obtain $(z^*,\mu^*)$
\For{$i \notin \overline{\mathcal{O}}$}
\State $\Tilde{r}_i \leftarrow u_{T(\ear),i} + \sum_{l \notin i} u_{T(\ear),l} - V_{T(\ear)}^\text{DFA}\left(S_0\right) - \sum_{l \in i} \mu_l^* - \mu^*_{K_s}$
\EndFor
\State $i^* \leftarrow \argmax_{i \notin \overline{\mathcal{O}}} \tilde{r}_i$
\If{$\tilde{r}_i^* > 0$}
\State $r_{i^*} \leftarrow V_{T(\ear)}^\text{DFA}\left(S_{i^*}\right) - V_{T(\ear)}^\text{DFA}\left(S_{0}\right)$
\State $\overline{\mathcal{O}} \leftarrow \overline{\mathcal{O}} \cup \left\{i^*\right\}$
\EndIf
\doWhile{$\tilde{r}_i^* > 0$ and $|\overline{\mathcal{O}}| < |\mathcal{L}| + N_\text{gen}$}
\State Compute $\mathcal{S} =$ top $N_\text{eval}$ solutions of $\left(\mathcal{P}_{IO}\right)$ restrained to $\overline{\mathcal{O}}$
\State \Return $\argmax_{S \in \mathcal{S}} V_{T(\ear)}^\text{DFA}(S)$
\end{algorithmic}
\end{algorithm}

The complexity of the first loop of Algorithm \ref{alg:bld_alg} is $O \left(|\mathcal{O}| \cdot |\Omega| \cdot \ear\right)$. As $|\mathcal{O}| \simeq L^{K_b}$, this loop is the theoretical bottleneck of the algorithm. However, it can be easily parallelized, making it less computationally expensive than the while loop. The master problem in the while loop is easy to solve since it has only $\overline{\mathcal{O}}$ variables and can use the solution of the previous iteration as a warm start. The index $i^*$ can be computed efficiently using a MILP. Finally, the practical bottleneck of the algorithm is the computation of $V_{T(\ear)}^\text{DFA}\left(S_{i^*}\right)$ whose complexity is $O \left(L^2 \cdot |\Omega| \cdot \ear\right)$. We note, however, that the quality of the bounds increases with $\ear$, making $\tilde{r}$ a better approximation of $\overline{r}$, which in turn improves the quality of the bundles generated. Therefore, although the complexity of each iteration increases linearly in $\ear$, algorithm \ref{alg:bld_alg} generally requires fewer iterations to produce high-quality bundles as $\ear$ increases. As a result, algorithm \ref{alg:bld_alg} is able to generate high-quality sets of options in a tractable manner for a wide range of values of $\ear$.

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.7\linewidth]{media/BundlingAlg.png}
% \caption{Bundling Algorithm Diagram} \label{fig:bld_alg_diagram}
% \end{figure}

% \begin{algorithm}
%\footnotesize

% \caption{Static Bundling Algorithm}\label{static_bundling_algorithm}
% \begin{algorithmic}
% \Require $\mathcal{L}$: set of products
% \For{$b \in \mathcal{B}(\mathcal{L})$}
%     \State $u_b \leftarrow \texttt{optimistic\_upper\_bound}(b)$
% \EndFor
% \State $\mathcal{S} = \texttt{sorted\_sets}(\mathcal{P}(\mathcal{L}), u)$ \Comment{sort feasible sets of options by decreasing upper bound}
% \State $U^* = U_{\mathcal{S}_{0}}$ 
% \State $L^* = -\infty$
% \For{$S \in \mathcal{S}$}
%     \If{$U_{S} \leq L^*$}
%         \State \texttt{STOP}
%     \EndIf
%     \State $L_{S} \leftarrow \texttt{DFA}(S)$
%     \If{$L_{S} > L^*$}
%         \State $L^* \leftarrow L_{S}$
%         \State $S^* \leftarrow {S}$
%     \EndIf
% \EndFor
% \State \Return $S^*, L^*, U^*$
% \end{algorithmic}

% \end{algorithm}

==> 6_Computational_Results.tex <==
\section{Computational Results and Industry-Driven Case Study} \label{section:ExperimentalResults}

To evaluate the performance of the DFA and the Robust Bundle Algorithm, we conducted numerical experiments on synthetic and real data. In Section \ref{section:synthetic_experiments}, we compare the bounds of section \ref{section:bounds} against other approximations on synthetic data allowing us to evaluate the performance of the bounds in a wide range of scenarios. Further, we analyze the potential of bundling and the effectiveness of our proposed bundling algorithm for different customer utility functions. Section \ref{section:real_world_experiments} analyzes the performance of our bundling algorithm on a real-world case study and compares it to in-use industry solutions. Algorithm \ref{alg:bld_alg} achieves up to 12\% guaranteed lower cost and 14-18\% less empty miles compared to the \say{no bundle} solution, as well as a significant worst-case cost reduction for comparable empty miles in comparison to the industry solution.

\subsection{Synthetic data experiments}\label{section:synthetic_experiments}

We generate a synthetic dataset by creating items described by two intrinsic qualities \textit{a} and \textit{b} i.e. item $j$ is described by $q_{j,a}$ and $q_{j,b}$. We assume the intrinsic qualities of all items to be independent and uniformly distributed following a standard uniform distribution. Each type of customer $\omega$ attributes a perceived quality $q_i^\omega$ to option $i$. The perceived quality depends on $\beta$, the quality sensitivity shares across all customer types, and a function $g^\omega$ such that the perceived quality of option $i$ for a customer of type $\omega$ is given by:
$$q_i^\omega \triangleq \beta \cdot g^\omega(q_{j_1,a}, q_{j_1,b},\hdots,q_{j_n,a}, q_{j_n,b}), \quad j_1,\hdots,j_n \in i$$
Note that the ordering of items in a bundle can affect its perceived quality.

In the two following subsections, we consider two types of customers each having the same probability of arrival $\left(\mathbb{P}_1 = \mathbb{P}_2 = 0.5\right)$ and set the arrival rate to $\arate = 0.1$.

\subsubsection{Bounds performance}\label{subsubsection:bound_perf}\hfill

We compare here the performance of the bounds developed in section \ref{section:bounds} to the fluid and static approximations given in the Supplementary Material section. We consider two types of customers. Type 1 values the intrinsic quality \textit{a} more than the intrinsic quality \textit{b}, whereas type 2 does the contrary:
\begin{align*}
    q_i^1 &\triangleq \beta \left(\sum_{j \in i} q_{j,a} + \frac{1}{2} \sum_{j \in i} q_{j,b}\right)\\
    q_i^2 &\triangleq \beta \left(\frac{1}{2} \sum_{j \in i} q_{j,a} + \sum_{j \in i} q_{j,b}\right)
\end{align*}
We vary the number $L$ of items generated, the quality sensitivity $\beta$, and the horizon $T$ to observe the performance for 1,3 and 10 expected arrivals per item. All items are offered as a single item option. Table \ref{tab:bounds_perf} reports the relative optimality gap of the static approximation $V^S$, the lower bound $V^L$, and the DFA bound $V^\text{DFA}$, averaged over 50 runs. We remark that $V^S$ and $V^L$ perform similarly when the demand per item is small. However, $V^L$ outperforms $V^S$ as the demand increases. The DFA bound performs similarly to two other bounds when $L=1$ and $\ear / L = 1$, which corresponds to an extremely short season. For the remaining cases, the DFA bound performs significantly better. In particular, the performance of the DFA bound improves as $\ear$ increases (or equivalently, as $L$ increases with $\ear / L$ fixed) whereas $V^L$ mostly improves as $\ear / L$ increases.

\begin{table}[h]
\centering
\resizebox{0.75\textwidth}{3cm}{
\small
% \begin{tabular}{ll|lll|lll|lll}
% \toprule
%   & {} & \multicolumn{3}{l}{Static gap ratio} & \multicolumn{3}{l}{$V^L$ gap ratio} & \multicolumn{3}{l}{DFA gap ratio} \\
%   & $\arate T/L$ &                1 &        3 &       10 &             1 &       3 &      10 &          1 &       3 &      10 \\
% \cline{0-1} $L$ & $\beta$ &                  &          &          &               &         &         &            &         &         \\
% \midrule
% 1 & 0.1  &           1.29 &  2.89 &  4.70 &        1.23 &  2.47 &  2.73 &     0.91 &  0.50 &  0.12 \\
%   & 1.0  &           1.98 &  4.02 &  5.61 &        1.89 &  3.48 &  3.28 &     1.10 &  0.65 &  0.17 \\
%   & 10.0 &           6.24 &  7.95 &  6.37 &        6.25 &  7.33 &  3.66 &     \underline{8.11} &  5.13 &  0.98 \\\hline
% 3 & 0.1  &           4.21 &  7.14 &  7.62 &        4.03 &  6.16 &  4.40 &     2.13 &  0.55 &  0.08 \\
%   & 1.0  &           5.65 &  8.67 &  8.20 &        5.44 &  7.57 &  4.76 &     2.22 &  0.65 &  0.11 \\
%   & 10.0 &           14.58 &  12.63 &  7.39 &        14.69 &  11.66 &  4.18 &     7.91 &  2.79 &  0.30 \\\hline
% 5 & 0.1  &           6.07 &  8.61 &  8.00 &        5.75 &  7.15 &  4.08 &     1.80 &  0.40 &  0.06 \\
%   & 1.0  &           7.76 &  9.90 &  8.34 &        7.41 &  8.30 &  4.26 &     1.85 &  0.50 &  0.07 \\
%   & 10.0 &           16.99 &  11.96 &  7.02 &        17.00 &  10.50 &  3.43 &     6.96 &  1.61 &  0.16 \\
% \bottomrule
% \end{tabular} 
\begin{tabular}{ll|lll|lll|lll}
\toprule
  & {} & \multicolumn{3}{l}{$V^S$ gap ratio} & \multicolumn{3}{l}{$V^L$ gap ratio} & \multicolumn{3}{l}{DFA gap ratio} \\
  & $\ear/L$ &                1 &        3 &       10 &             1 &       3 &      10 &          1 &       3 &      10 \\
\cline{0-1} $L$ & $\beta$ &                  &          &          &               &         &         &            &         &         \\
\midrule
1 & 0.1  &           0.0132 &  0.0294 &  0.0475 &        0.0125 &  0.0251 &  0.0275 &     0.0094 &  0.0052 &  0.0012 \\
  & 1.0  &           0.0232 &  0.0452 &  0.0595 &        0.0223 &  0.0393 &  0.0350 &     0.0130 &  0.0069 &  0.0014 \\
  & 10.0 &           0.0842 &  0.0960 &  0.0631 &        0.0850 &  0.0908 &  0.0373 &     0.0757 &  0.0474 &  0.0094 \\\hline
3 & 0.1  &           0.0428 &  0.0722 &  0.0766 &        0.0409 &  0.0624 &  0.0442 &     0.0216 &  0.0055 &  0.0008 \\
  & 1.0  &           0.0636 &  0.0935 &  0.0841 &        0.0615 &  0.0821 &  0.0490 &     0.0244 &  0.0069 &  0.0010 \\
  & 10.0 &           0.1718 &  0.1352 &  0.0708 &        0.1742 &  0.1265 &  0.0407 &     0.0838 &  0.0277 &  0.0029 \\\hline
5 & 0.1  &           0.0615 &  0.0868 &  0.0802 &        0.0583 &  0.0721 &  0.0409 &     0.0182 &  0.0040 &  0.0006 \\
  & 1.0  &           0.0855 &  0.1043 &  0.0846 &        0.0820 &  0.0880 &  0.0433 &     0.0199 &  0.0052 &  0.0006 \\
  & 10.0 &           0.1918 &  0.1221 &  0.0663 &        0.1928 &  0.1087 &  0.0329 &     0.0736 &  0.0159 &  0.0015 \\\hline
8 & 0.1  &           0.0765 &  0.0863 &  0.0765 &        0.0701 &  0.0626 &  0.0287 &     0.0096 &  0.0020 &  0.0002 \\
  & 1.0  &           0.1009 &  0.0974 &  0.0786 &        0.0936 &  0.0715 &  0.0295 &     0.0113 &  0.0025 &  0.0002 \\
  & 10.0 &           0.1731 &  0.0916 &  0.0584 &        0.1697 &  0.0693 &  0.0206 &     0.0462 &  0.0062 &  0.0007 \\
\bottomrule
\end{tabular} 
}
\caption{Comparison of the relative optimality gap of the DFA against the static approximation and worst-case lower bound.}
\label{tab:bounds_perf}
\end{table}

Figure \ref{fig:bounds_comparison} shows the performance of the bounds of section \ref{section:bounds} in addition to the static ($V^S$) and fluid ($V^F$) approximations for $L = 5$, $\beta = 10$, and either no salvage value (\ref{fig:bounds_no_penalty}) or a positive salvage value identical to all items (\ref{fig:bounds_penalty}). We observe that, although largely dominated by $V^F$ for $T$ taking small values, $V^U$ quickly becomes the tightest upper bound. In particular, unlike $V^F$, $V^U$ converges to $V^*$ independently of the salvage values. The lower bounds perform similarly for $T$ small. As $T$ increases, $V^\text{DFA}$ converges rapidly to $V^*$ whereas the optimality gap of $V^S$ and $V^L$ remains significant.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/bounds_illustration.pdf}
        \caption{$\xi_i = 0, \quad \forall i \in \mathcal{O}$}
        \label{fig:bounds_no_penalty}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/bounds_illustration_penalty.pdf}
        \caption{$\xi_i = 100, \quad \forall i \in \mathcal{O}$}
        \label{fig:bounds_penalty}
    \end{subfigure}
    \caption{Performance comparison between the bounds of section \ref{section:bounds} (blue) and the fluid and static approximations (orange). In figure \ref{fig:bounds_no_penalty}, options have no salvage value. In figure \ref{fig:bounds_penalty}, all options have a salvage value of 6.}
    \label{fig:bounds_comparison}
\end{figure}

Those results suggest that $V^U$ and $V^\text{DFA}$ are a great choice of upper and lower bounds on the expected revenue when the number of expected arrivals per item is not too small.

\subsubsection{Bundling algorithm performance}\label{subsubsection:bdl_perf}\hfill

We now compare the revenue improvement from bundling in three scenarios (A), (B), and (C). For all scenarios, the perceived quality of option $i$ for customer type 1 is:
\begin{align*}
    q_i^1 &\triangleq \frac{\beta}{2} \left(\sum_{j \in i} q_{j,a} + \sum_{j \in i} q_{j,b}\right)
\end{align*}
Depending on the scenarios, the perceived quality of option $i$ for customer type 2 is either:
\begin{align*}
    q_i^2 &\triangleq \beta \sum_{j \in i} q_{j,a} \tag{A}\\
    q_i^2 &\triangleq 2\beta \cdot \min\left\{\sum_{j \in i} q_{j,a}, \sum_{j \in i} q_{j,b}\right\} \tag{B}\\
    q_i^2 &\triangleq \beta \left(\sum_{j \in i} q_{j,a}\right)^{\frac{3}{2}} \tag{C}
\end{align*}
Namely, customer type 1 values the average of the intrinsic qualities $a$ and $b$. Customer type 2 (A) only values the intrinsic quality $a$. Customer type 2 (B) values double the minimum between the intrinsic quality of $a$ and $b$. Finally, Customer type 2 (C) values the intrinsic quality $a$ with a superlinear rate.

Figure \ref{fig:bundling_algorithm_perf} highlights the structure of the set of options returned by the bundling algorithm in different scenarios as a function of the horizon $T$. We observe in all three scenarios that the proportion of items part of a bundle is large ($\geq 80\%$) when the horizon is small. This results from the fact that the perceived quality of a bundle is generally larger than the individual perceived quality of each item it contains. Hence when the horizon is too short to guarantee to sell all items, bundling allows one to increase the perceived quality of the offered options and thus increases short-horizon revenue. We also remark that in all three scenarios, the number of items offered as a single item option increases steadily with the horizon $T$. Combined with figure \ref{fig:dfa_improvement} showing the relative improvement of the DFA bounds resulting from suggesting the options of Algorithm \ref{alg:bld_alg} instead of single items only, this observation is consistent with the discussion in Section \ref{section:DP} regarding the decreasing revenue improvement of bundling as $T$ grows. This is particularly apparent in scenario (A), where bundles are no longer offered after $T \simeq 300$. However, we see that bundles remain desirable for much longer horizons in scenarios (B) and (C). While the total perceived quality is not affected by bundling in scenario (A), the perceived quality function of customer type 2 allows bundling to increase total perceived quality in scenarios (B) and (C). Specifically, scenario (B) profits from bundles of sizes 2 and 3 by grouping items with low intrinsic quality $b$, and scenario (C) profits considerably from bundles of size 3 by grouping items with high intrinsic quality $a$. We conclude that although the gains from bundling are short-lived when bundles cannot affect the total perceived quality of the proposed options, bundling remains valuable for longer horizons when such perceived quality improvements are achievable.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/size_distrib.pdf}
        \caption{}\label{fig:size_distrib}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/dfa_improvement.pdf}
        \caption{}\label{fig:dfa_improvement}
    \end{subfigure}
    \caption{Solution structure and performance for different customers perceived quality function, averaged over 50 runs with $L = 10$. Figure \ref{fig:size_distrib} shows the proportion of items part of an option of size 1 (dotted), 2 (dashed), or 3 (solid). Figure \ref{fig:dfa_improvement} shows the relative DFA improvement $\frac{V^\text{DFA}\left(S_\text{BA(3)}\right)-V^\text{DFA}(S_0)}{V^\text{DFA}(S_0)}$ where $S_\text{BA(3)}$ is the solution of the bundling algorithm for $K_b = 3$ and $S_0$ is the \say{no bundle} set of options.} \label{fig:bundling_algorithm_perf}
\end{figure}

Finally, we analyze the efficiency of the bundling algorithm to generate bundles. Recall that Algorithm $\ref{alg:bld_alg}$ uses perturbed reduced costs $\tilde{r}$ instead of the exact reduced costs $\overline{r}$. The accuracy of $\tilde{r}$ improves as the gap between $V^\text{DFA}$ and $V^U$ decreases, so one can expect Algorithm $\ref{alg:bld_alg}$ to perform better for $T$ taking large values following the result obtained in \ref{subsubsection:bound_perf}. Figure \ref{fig:lp_obj} shows the proportion of the optimal objective of $\left(\mathcal{P}_{LP}\right)$ achieved by the objective value of the master problem as the number of generated bundle increases. The objective improvement is the slowest for $T=100$ reported in figure \ref{fig:lp_obj_1}. We observe that the objective improvement is faster in scenarios (B) and (C) where some bundles have a significant edge over others. Nevertheless, a large proportion of the optimal objective is achieved with a small number of bundles generated in all three scenarios, suggesting that Algorithm 1 is able to generate high-quality bundles rapidly even when the bounds are not tight. We see in figure \ref{fig:lp_obj_3} that the objective improvement is faster for $T = 300$, reflecting the fact that $\tilde{r}$ provides a better approximation of $\overline{r}$ as $T$ increases.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/lp_obj_1.pdf}
        \caption{$T = 100$}\label{fig:lp_obj_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/lp_obj_3.pdf}
        \caption{$T = 300$}\label{fig:lp_obj_3}
    \end{subfigure}
    \caption{Evolution of the ratio of the objective of the master problem to the objective of $\left(\mathcal{P}_{LP}\right)$ for horizons $T=100$ and $T=300$. The solid line represents the average taken over 100 runs, and the envelope contains 95\% of the trajectories.}
    \label{fig:lp_obj}
\end{figure}

\subsection{Decentralized and Non-Dedicated Fleet Operations in the Freight Industry} \label{section:real_world_experiments}

We now present the analysis of a digital freight brokerage platform. On one side, shippers provide \textit{loads} (items) consisting of a single shipment associated with an origin-destination pair. On the other side, carriers arrive on the platform, observe the option-price pairs presented by the platform, and decide to select one of the options or leave the platform. The objective of the platform is to form a set of options and dynamically price each of them to minimize its operational costs, or equivalently, maximize the opposite of the revenue.

The dataset covers 2.424 loads in the Texas triangle, with specified pick-up and drop-off locations, supplied to the platform over 2.5 months. Historical loads are represented in figure $\ref{fig:historical_loads}$. 

\begin{figure}[h]
\centering
\makebox[\textwidth][c]{\includegraphics[scale=0.5]{media/historical_loads.png}}
\caption{Historical loads, blue and red dots represent pick-up and drop-off locations, respectively.}
\label{fig:historical_loads}
\end{figure}

The space is divided into 4 markets denoted by their major cities: San Antonio, Austin, Dallas, and Houston. We denote by $\Omega$ the set of markets. Each load has an origin and destination market, defined as the city closest to the pick-up and drop-off locations. We are provided with the average carrier arrival rate in each market and assume that carriers arrive in the center of major cities. We note that the distribution of arrivals across markets is similar to the distribution of loads pick-up and drop-off locations, as can be seen in Table \ref{table:loads_carriers_distribution}. We also remark that the two less active markets, San Antonio and Austin, only account for $17\%$ of arrivals.
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{|c|c|c|c|c|}
        \cline{2-5}
        \multicolumn{1}{c|}{} & \textbf{San Antonio} & \textbf{Austin} & \textbf{Dallas} & \textbf{Houston}\\
        \hline
        {Pickup} & 11.3\% & 5.53\% & 45.0\% & 38.2\%\\
        {Dropoff} & 12.5\% & 8.6\% & 40.1\% & 38.9\% \\
        {Carrier arrivals} & 11\% & 6\% & 45\% & 38\%\\
        \hline
    \end{tabular}
    \caption{Loads and carrier distributions.}
    \label{table:loads_carriers_distribution}
\end{table}

Finally, we have access to a MNL model calibrated on empirical data from our industrial partner. This model includes the price sensitivity $\beta_p$ and the following parameters:
\begin{itemize}
    \item $\beta_0$: MNL constant
    \item $\beta_d$: in-load distance sensitivity
    \item $\beta_{e}$: empty miles sensitivity
    \item $\beta_{\texttt{b2}}$ and $\beta_{\texttt{b3}}$: carrier aversion for bundles of size 2 and 3
    \item $\forall \omega \in \Omega$, $\beta_{\texttt{org}}(\omega)$ and $\beta_{\texttt{dst}}(\omega)$: market preferences
\end{itemize}
The perceived quality of option $i$ for a carrier arriving in market $\omega$ is then computed as follows:
$$q_i^\omega = \beta_0 + \beta_d d_i + \beta_{e} e_i^\omega + \beta_{\texttt{b2}} \mathds{1}_{\{\#i=2\}} + \beta_{\texttt{b3}} \mathds{1}_{\{\#i=3\}} + \beta_{\texttt{org}}(i_\texttt{org}) + \beta_{\texttt{dst}}(i_\texttt{dst})$$
where $d_i$ is the total in-load distance of option $i$, $e_i^\omega$ is the total empty miles from delivering option $i$ starting from market $\omega$, and $i_\texttt{org}$ and $i_\texttt{dst}$ are respectively the origin and destination markets of option $i$.

We consider 1-day seasons: a set containing the average daily number of loads ($L = 32$) is fixed at the beginning of the season, bundles are formed, and additional loads provided by shippers during the season are ignored. We set $\arate = 0.1$ and fix $T$ such that $\ear$ matches the daily number of arrivals. At the end of the season, unmatched loads are salvaged for a cost of $1+\alpha$ times the average historical cost of loads with corresponding origin-destination market pair. We choose $\alpha$ empirically so that the total expected cost over a season, obtained by suggesting individual loads only, matches the historical daily cost of the platform.

To gain some insight into the solutions produced by our algorithm, we first study a simple example with 10 loads randomly sampled from the historical loads and a medium bundle aversion. Figure \ref{fig:bdl_alg} shows the bundle generated by our algorithm for varying demand levels before the end of the season and different values of $N_\text{eval}$.
Figures \ref{fig:bdl_alg_1} and \ref{fig:bdl_alg_2} show the importance of the last step of the Bundling Algorithm. With $N_\text{eval} = 1$, the selected options are those minimizing the total individual cost improvements. This results in the set of options \{\texttt{2}, \texttt{5-4-6}, \texttt{9-1-7}, \texttt{0-3-8}\} with 3 bundles starting in the market of Dallas, and none in the market of Houston. This solution is suboptimal since carriers arriving in Houston have no attractive option resulting in an important loss of resources. In contrast, a larger value of $N_\text{eval}$ allows the interaction between options to be addressed by evaluating multiple high-potential sets of options. Indeed, $\ref{fig:bdl_alg_2}$ shows that the solution produced with $N_\text{eval} = 10$ is more balanced than the one previously observed, with a bundle starting in each of the two largest markets (\texttt{0-3-8} and \texttt{7-9-2}), a third starting near the two smallest markets (\texttt{1-4-5}), and a single load starting in the largest market (\texttt{6}). This selection of options is therefore preferable, as the platform is more likely to match every options to a carrier before the end of the season.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/triangle_sample_1.png}
        \caption{$\ear/L = 1$, $N_\text{eval} = 1$}
        \label{fig:bdl_alg_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/triangle_sample_2.png}
        \caption{$\ear/L = 1$, $N_\text{eval} = 10$}
        \label{fig:bdl_alg_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/triangle_sample_3.png}
        \caption{$\ear/L = 5$, $N_\text{eval} = 10$}
        \label{fig:bdl_alg_3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/triangle_sample_4.png}
        \caption{$\ear/L = 10$, $N_\text{eval} = 10$}
        \label{fig:bdl_alg_4}
    \end{subfigure}
    \hfill
    \raggedright
    \begin{subfigure}{0.8\linewidth}
        \includegraphics[width=\linewidth]{media/triangle_sample_legend.png}
    \end{subfigure}
    \caption{Example results of the Algorithm \ref{alg:bld_alg} for a sample with $L = 10$. A different color represents each option.}
    \label{fig:bdl_alg}
\end{figure}

The two first subfigures \ref{fig:bdl_alg_1} and \ref{fig:bdl_alg_2} correspond to high-stress scenarios $\ear/L = 1$ i.e. an demand equal to the number of loads. In this case, as highlighted in \ref{subsubsection:bdl_perf}, bundles are highly valuable as, in addition to reducing empty miles, they significantly increase the likelihood of matching all loads before the season ends. As the demand increases, the short-term value of bundles decreases and, assuming a medium bundle aversion, the perceived quality improvement from bundling is limited resulting in few bundles selected by Algorithm \ref{alg:bld_alg}. For $\ear/L = 5$, two bundles of size 3 (\texttt{0-3-8} and \texttt{4-9-2}) are selected, but only one bundle of size 2 (\texttt{3-8}) is selected for $\ear/L = 10$. The intuitive reasons why \texttt{3-8} remains valuable for a large demand are (i) the drop-off location of \texttt{3} is closer than any city to the pick-up location of \texttt{8}, and (ii) the closest city to the pick-up location of \texttt{8} is Austin, the city with the smallest arrival rate and market preference $\beta_\texttt{org}$.

We evaluate the performance of the sets of options returned by Algorithm \ref{alg:bld_alg} with option size limited to 2 ($S_\text{BA(2)}$) and 3 ($S_\text{BA(3)}$) and compare them to the \say{no bundle} set $S_0$ and the industry solution $S_\text{EM}$. The latter set consists of options of size at most 2 minimizing the expected empty miles, obtained by solving the linear program $\left(\mathcal{P}_\text{EM}\right)$ given in the Supplementary Material section.

Table \ref{tab:avg_costs_bdl_aversion} and figure \ref{fig:avg_costs_bdl_aversion} report the DFA and upper bound $V^U$ of those 4 candidates averaged over 50 seasons. In addition, table \ref{tab:avg_costs_bdl_aversion} gives the upper bound of the sets $S_2^*$ and $S_3^*$ that maximize $V^U$ with options of size at most 2 and 3, respectively. In the absence of bundle aversion, the upper bound of set $S_0$ is dominated by the DFA bound of all other sets. The set $S_\text{BA(3)}$ performs best with a guaranteed 12\% decrease in cost compared to $S_0$. The bounds of $S_\text{BA(2)}$ dominate those of $S_\text{EM}$, although the gap between lower and upper bounds is too large to guarantee a cost reduction from choosing $S_\text{BA(2)}$ over $S_\text{EM}$. As the bundle aversion increases, the cost of all solutions including bundles increases: the set $S_\text{BA(3)}$ only guarantees a 0.5\% cost decrease over set $S_0$ with medium bundle aversion, and does not guarantee a cost reduction when bundle aversion is high. Still, the DFA bound of $S_\text{BA(3)}$ dominates the one of $S_0$ by 4.8\% with medium bundle aversion. Further, the DFA bound of $S_\text{BA(2)}$ and $S_\text{BA(3)}$ are always greater than the one of $S_0$, unlike $S_\text{EM}$ whose bounds become dominated by those of $S_0$ when bundle aversion is high. This results from the fact that problem $\left(\mathcal{P}_\text{EM}\right)$ does not take into account carrier preferences.

\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{\small
\begin{tabular}{l|llll|llllll}
\toprule
 & \multicolumn{4}{c}{$-V^\text{DFA}$} & \multicolumn{6}{c}{$-V^U$} \\
Bundle aversion &            $S_0$ &  $S_{\text{BA}(2)}$ &  $S_{\text{BA}(3)}$ & $S_\text{EM}$ &   $S_0$ &  $S_{\text{BA}(2)}$ &  $S_{\text{BA}(3)}$ & $S_\text{EM}$ &  $S^*_2$ &  $S^*_3$ \\
\midrule
none &            16644 &       14993 &       14053 &    15197 &   15913 &       14426 &       13651 &    14624 &  14417 &  13624 \\
low &            16644 &       15687 &       15008 &    15879 &   15913 &       15171 &       14633 &    15362 &  15155 &  14617 \\
medium &            16644 &       16246 &       15845 &    16522 &   15913 &       15715 &       15500 &    16067 &  15660 &  15447 \\
high &            16644 &       16525 &       16422 &    17117 &   15913 &       15883 &       15946 &    16728 &  15845 &  15815 \\
\bottomrule
\end{tabular}
}
\caption{Average costs for various bundle aversion levels, lower is better.}
\label{tab:avg_costs_bdl_aversion}
\end{table}

\begin{figure}[h]
\centering
\makebox[\textwidth][c]{\includegraphics[scale=0.7]{media/expected_costs_aversion.pdf}}
\caption{Expected costs for different levels of bundle aversion. For each set of options, solid lines indicate the lower bound provided by the DFA and dashed lines indicate the upper bound.}
\label{fig:avg_costs_bdl_aversion}
\end{figure}

Finally, figure \ref{fig:estimated_empty_miles} shows the estimated empty miles resulting from suggesting the 4 candidate sets. The estimation assumes that each option will be delivered starting from the city of its origin market. We observe that the sets $S_\text{BA(2)}$ and $S_\text{BA(3)}$ yield fewer estimated empty miles than $S_0$ for any bundle aversion level, with $S_\text{BA(3)}$ achieving a 14-18\% decrease in estimated empty miles. Although the set $S_\text{EM}$ obtains the lowest estimated empty miles, we note that those obtained by $S_\text{BA(3)}$ are comparable while achieving significantly lower costs. This result indicates that, despite lower empty miles and higher carrier utility being positively correlated, minimizing empty miles does not yield minimum operating costs, and taking into account carrier spatial distribution and preferences can further reduce costs.

\begin{figure}[h]
\centering
\makebox[\textwidth][c]{\includegraphics[scale=0.7]{media/estimated_empty_miles.pdf}}
\caption{Expected empty miles for different levels of bundle aversion.}
\label{fig:estimated_empty_miles}
\end{figure}
